Using Simulated Data to Generate Images of Climate Change

Generative adversarial networks (GANs) used in domain adaptation tasks have the ability to generate images that are both realistic and personalized, transforming an input image while maintaining its identifiable characteristics. However, they often require a large quantity of training data to produce high-quality images in a robust way, which limits their usability in cases when access to data is limited. In our paper, we explore the potential of using images from a simulated 3D environment to improve a domain adaptation task carried out by the MUNIT architecture, aiming to use the resulting images to raise awareness of the potential future impacts of climate change.

==> notes.tex <==
Climate change and the transition to a lower carbon economy–policy, legal, regulatory, technology and market change related to the issue of climate change could increase costs, reduce demand for our products, reduce revenue and limit certain growth opportunities.\\
To help anticipate greater regulatory requirements affecting our GHG emissions, we use a carbon cost when evaluating our plans for large new projects and those for which emissions costs would be a material part of the project. In industrialized countries, this is currently \$40 per tonne of CO2 equivalent, and we also stress test at a carbon price of \$80 per tonne.

a report by banking giant HSBC, major firms like BP and Shell could lose up to 60 percent of their market values if countries pass tough carbon regulations that force oil giants to keep some of their fossil reserves in the ground.

\begin{table}[h!]
\caption{Number of Companies per Sector in S\&P 500.}
\label{sp500}
\vskip 0.12in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
GIS Sector & Number of Companies \\
\midrule
Consumer Products & $\ 33$ \\
Real Estate & $\ 32$ \\
Oil and Gas   &$\ 29$ \\
Utilities & $\ 28$ \\
Materials & $\ 26$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Other initiatives:
https://climatedisclosure100.info/

https://www.fsb-tcfd.org/
https://www.cdp.net/en/research



